Functorial evolution of quantum fields

We present a compositional algebraic framework to describe the evolution of quantum fields in discretised spacetimes. We show how familiar notions from Relativity and quantum causality can be recovered in a purely order-theoretic way from the causal order of events in spacetime, with no direct mention of analysis or topology. We formulate theory-independent notions of fields over causal orders in a compositional, functorial way. We draw a strong connection to Algebraic Quantum Field Theory (AQFT), using a sheaf-theoretical approach in our definition of spaces of states over regions of spacetime. We introduce notions of symmetry and cellular automata, which we show to subsume existing definitions of Quantum Cellular Automata (QCA) from previous literature. Given the extreme flexibility of our constructions, we propose that our framework be used as the starting point for new developments in AQFT, QCA and more generally Quantum Field Theory.

==> packages.tex <==
%% MATHS %%
\usepackage{mathtools} % Loads and extends amsmath
\usepackage{amstext} % Skimpy version to load when writing for IOP (which disallows amsmath)
\usepackage{amssymb} % Extram mathematical symbols (loads amsfonts)
\usepackage{bbold} % Sans-serif blackboard bold font for numbers
\usepackage{amsthm} % Theorem environments
\usepackage{stmaryrd} % Some maths symbols for logic and computer science
%\usepackage{cjhebrew} % Jewish symbols
%\usepackage[nodisplayskipstretch]{setspace} % Redefines spacing before/after equations

%% INPUT %%
%\usepackage[applemac]{inputenc} % Support for non-standard characters from macbook keyboard
\usepackage[utf8]{inputenc}
%\usepackage[italian]{babel} % Support for italian accented characters

%% WRITING %%
\usepackage{relsize} % Additional relative sizes for fonts
\usepackage{microtype} % Improves appearance of writing
\usepackage{fullpage} % Reduces lateral page margins for vanilla classes
%\usepackage{multicol} % Multi-column environments
\usepackage{csquotes} % Environments for quotes
%\usepackage{fancyvrb} % Verbatim environments
\usepackage{ragged2e} % (I don't remember what this does)
%\usepackage{enumerate} % Macros for enumerate environments
\usepackage{cancel}
\usepackage{pifont}

%% CITATIONS %%
\usepackage{hyperref} % Hyperlink citations, comment out for arxiv submission 
% \usepackage[nocompress]{cite} % Comment out if using natbib or apacite
% \usepackage[compress]{cite} % Comment out if using natbib or apacite
% \usepackage[sort&compress]{natbib} % Comment out if using cite or apacite
%\usepackage[round,authoryear,sort&compress]{natbib} % Comment out if using cite or apacite
% \usepackage{apacite} % Comment out if using natbib or cite

%% GRAPHICS %%
\usepackage{graphicx} % Import of graphics
%\usepackage{subcaption} % Captioning and referencing sub-figures
\usepackage[usenames,dvipsnames]{xcolor} % Introduces colour names
\usepackage{stackengine}
\usepackage{tikz} % TikZ
\usepackage{circuitikz} % TikZ circuit diagrams 
% \usepackage{tikzfig} 
\usetikzlibrary{
	arrows,
	shapes,
	decorations,
	intersections,
	backgrounds,
	positioning,
	circuits.ee.IEC
	}
% \usepackage{tikzit}
\usepackage{tikz-cd}

\usepackage{rotating}
\usepackage{floatpag}
\usepackage{xifthen}
\usepackage[normalem]{ulem}

%IDENTITY MAP%
\usepackage{dsfont}



